Event-triggered and distributed model predictive control for guaranteed collision avoidance in UAV swarms

Distributed model predictive control (DMPC) is often used to tackle path planning for unmanned aerial vehicle (UAV) swarms. However, it requires considerable computations on-board the UAV, leading to increased weight and power consumption. In this work, we propose to offload path planning computations to multiple ground-based computation units. As simultaneously communicating and recomputing all trajectories is not feasible for a large swarm with tight timing requirements, we develop a novel event-triggered DMPC that selects a subset of most relevant UAV trajectories to be replanned. The resulting architecture reduces UAV weight and power consumption, while the active redundancy provides robustness against computation unit failures. Moreover, the DMPC guarantees feasible and collision-free trajectories for UAVs with linear dynamics. In simulations, we demonstrate that our method can reliably plan trajectories, while saving 60% of network traffic and required computational power. Hardware-in-the-loop experiments show that it is suitable to control real quadcopter swarms.

==> event_triggered_dmpc_necsys22 - Kopie/Conclusion/Conclusion.tex <==
\section{Conclusions}
This paper presented an event-triggered path-planning algorithm for UAV swarms. The developed computation scheme selects a subset of UAVs and replans the trajectories of only these on stationary computation units. The DMPC based path planner guarantees recursive feasibility and collision free trajectories for linear UAV dynamics. Our approach has been demonstrated to reliably steer UAVs without any collisions.
% to their target positions. % when the number of \cus\ is much smaller than the number of UAVs. 
This shows that event-triggering can be used to lower the communications and computational resources needed for path planning while guaranteeing collision free trajectories. 
In future work, we will add static obstacle avoidance to ET-DMPC using a safe flight corridor (\cite{Park2020, Park2021}). Additionally, we will investigate distributed cooperative planners to avoid deadlocks.

%The choice of the event-trigger method has shown to be important for the performance of the system. Because the guarantees are independent of the trigger, it can be optimized freely without violating safety constraints. This opens the door to use machine learning to learn a trigger rule e.g. following \cite{LearningEventTriggeredControl} in future work. 

%In some scenarios, we noticed the occurrence of deadlocks. In future work, we will investigate the methods to avoid them, which were described in section \ref{sec:disc}. 
%Because the DSLPID-controller used in our experiments troubled to follow the generated trajectories, we will investigate methods, which allow to guarantee collision free trajectories for UAVs with nonlinear dynamics in the future.




% We introduced time variant BVC for collision avoidance, which are less conservative than classical BVC. It has been shown in simulation, that the number of computation nodes can be much smaller than the size of the UAV swarm to lead to suitable performance. The choice of the event-trigger has shown to be important for the performance of the system. Because the guarantees are independent of the trigger, it can be optimized freely without violating safety constraints. In future work, we will design an algorithm that learns this trigger based on \cite{LearningEventTriggeredControl}. 
 
%In order to ensure feasibility, the UAV has to stand still at the end of every planned trajectory. This limits the performance of the algorithm. This also means that the UAV needs the ability to hover over a position, which makes the algorithm not suitable for winged UAVs. Future work will focus on relaxing those constraints.

%We have showed that the algorithm works on a real world quadcopter swarm. However, we simulated the wireless communication network and the CUs. In a next step, we will implement the CUs in hardware and a wireless multi-hop network based on Mixer \cite{Mixer} through which the drones and computation nodes can communicate.

\section*{Acknowledgements}
We thank Sebastian Giedyk for his help with the development and implementation of the quadcopter testbed, Alexander von Rohr and Kurt Capellmann for their help with the execution of the simulations, and Christian Fiedler and Henrik Hose for feedback on the manuscript.

==> event_triggered_dmpc_necsys22 - Kopie/ET_DMPC/ET_DMPC.tex <==
\section{Event-triggered Distributed Model Predictive Control}
\begin{figure}
	\centering
	\subcaptionbox{Linearized constraints (\cite{Luis2019})}[.2\textwidth]{\includegraphics[width=.2\textwidth]{pictures/Luis.pdf}}
%\subcaptionbox{BVC}[.2\textwidth]{\includegraphics[width=.2\textwidth]{pictures/BVC.pdf}}\\
\subcaptionbox{TV-BVC (\cite{TVBVC})}[.2\textwidth]{\includegraphics[width=.2\textwidth]{pictures/TCBVC.pdf}}
\caption{Comparison of different anti-collision constraints for the trajectory at time $kT+T+\stimecol$. \capt{The colored areas specify the corresponding constraint of the trajectory with the same color. (a): Linearization of the constraints. There exists a set, where both trajectories can lie in. 
		%(b): Buffered Voroni Cells (BVC, \cite{Zhou2017}). Because the constraints are the same for the whole trajectory, it is more conservative (\cite{Luis2019}).
 (b): Time variant BVC (TV-BVC). The generated constraints restrict the allowed set of trajectories to separated sets. Here $d=||\ve{n}\uli{ij}\of{\stimecol+2T|(k-1)T}||_2$. %In contrast to classical BVC (\cite{Zhou2017}), these sets change with time.
}}
\label{fig:constrComp}
\end{figure}
In this section, we will now solve the three subproblems that we have defined in the section above.\\
{\bf Communication architecture.} The choice of the communication architecture is mainly influenced by related works (\cite{Zhou2017, Cai2018, Luis2019, Luis2020, Park2021}). To simplify the design of the DMPC and the ET, the algorithms should not have to deal with different timings and information states of the agents. Therefore, we choose a round based many-to-all architecture. During every round, it distributes all messages sent to all agents in the network. This synchronizes the agents, i.e they send/receive at the same time, and all agents have the same knowledge about the data sent in the network. From an implementation based point of view, this choice is reasonable too. There exist real world implementations of round based many-to-all architectures like Glossy (\cite{Ferrari2011}) or Mixer (\cite{Mixer}), which have been shown to meet the strict real-time and reliability requirements needed for fast control (\cite{FeedbackControlGoesWireless, PredictiveTriggering}). 

During the communication round, the UAVs send their current state and the \cus\ share their results of the path planning, which the corresponding UAVs and all \cus\ save in a buffer. 
After the communication round, the \cus\ decide which \cu\ replans the path of which UAV using ET. Because of the many-to-all protocol, every \cu\ has the same information and thus knows which UAV will be selected by the other \cus. This avoids the case of two \cus\ replanning the trajectory of the same UAV. Afterwards, each unit replans the trajectory of its chosen UAV. The maximum duration for the scheduling and replanning $T\ul{calc}$ is constant for every agent and time. A new communication round (length $T\ul{com}$) starts afterwards. The combined duration between the starts of two rounds is $T=T\ul{calc}+T\ul{com}$.

{\bf ET-DMPC.} The event trigger decides if during the $k$-th round, \cu\ $q$ replans the path of UAV $i$ ($\gamma\uli{q i}\of{k}=1$) or not ($\gamma\uli{q i}\of{k}=0$). Every \cu\ can only replan the path of one UAV in one round and every \cu\ should replan the path of a different UAV. 
%the following conditions have to hold for $\gamma\uli{p i}\of{k}\in\left\{0, 1\right\}$ and all $p\in\left[1, M\right], i\in\left[1, N\right]$:
%\begin{align*}
%&\sum_{q=1}^{M}\sum_{j=1}^{N} \gamma\uli{q j}\of{k} \leq M,~ \sum_{q=1}^{M}\gamma\uli{q i}\of{k} \leq 1,~ \sum_{j=1}^{N}\gamma\uli{p j}\of{k} \leq 1
%\end{align*}
 In this work, we use a priority based trigger rule (PBT) (\cite{PredictiveTriggering}), which we present at the end of this section, because it uses features from the DMPC, which we present next.

The control input for each UAV is piecewise-constant with sampling time $\stimes$ and horizon $h\ul{s}$
\begin{equation}
	\label{eq:discretisation}
		\veu\uli{i}\of{\tau+T|kT} = \sum_{\kappa=0}^{h\ul{s}-1}\Gamma\ul{\stimes}\of{\tau-\kappa\stimes}\veu\uli{i, \kappa|k},
\end{equation}
where $\Gamma\ul{\stimes}\of{t}$ is equal to $1$ for $0\leq t< \stimes$ and $0$ otherwise, and $\veu\uli{i, \kappa|k}$ are the time-discrete inputs. Additionally, we require $\tfrac{T}{\stimes} = \tfrac{h\ul{s}}{H}\in\mathbb{N}$ to ensure recursive feasibility of the following optimization problem with prediction horizon $H$ (\cite{Park2021}). When a \cu\ recalculates the trajectory of UAV $i$ at time $kT$, it solves the following optimization problem:
\begin{subequations}
	\label{eq:opt}
\begin{align}
	 \label{eq:objectfunc}
	\min_{\artinput\uli{i, \cdot|k} }\sum_{\kappa=0}^{h\ul{o}}\big[&||\vexset{i}\of{\kappa\stimeobj+T|kT}-\vex\uli{i, \mathrm{target}}||_{\ma{Q}\uli{i}}^2 \\&+ ||\veu\uli{i}\of{\kappa\stimeobj+T|kT}||_{\ma{R}\uli{i}}^2\big]\nonumber
\end{align}
%\begin{equation}
%	\label{eq:dynconst}
%	\text{s.t.~} 
%		\dot{\vex}\uli{i, set}\of{t|kT} = \ma{A}\uli{i}\vex\uli{i, set}\of{t|kT} + \ma{B}\uli{i}\vev\uli{i}\of{t|kT}
%	\end{equation}
%\begin{equation}
%	\label{eq:discretisation}
%		\vev\uli{i}\of{t|kT} = \sum_{\kappa=0}^{h_s}\sqcap\ul{T}\of{t-(kT+\kappa\stimes+T)}\vev\uli{i, \kappa},~ \frac{T}{\stimes} = \frac{h_s}{H}\in\mathbb{N}
%\end{equation}
\begin{align}
	\text{s.t.~}&\vex\uli{i}\of{\kappa\stimes+T+\delta|kT}\label{eq:dynconst}\\
	& = e^{\ma{A}\uli{i}(\kappa\stimes+\delta)}\vex\uli{i
	}\of{2T|(k-1)T}+\int_{0}^{\delta}e^{\ma{A}\uli{i}\tau}\ma{B}\uli{i}\diff\tau\artinput\uli{i, \kappa|k}\nonumber\\
	& + \sum_{\ell=0}^{\kappa-1}e^{\ma{A}\uli{i}((\kappa-\ell-1)\stimes+\delta)}\int_{0}^{\stimes}e^{\ma{A}\uli{i}\tau}\ma{B}\uli{i}\diff\tau\artinput\uli{i, \ell|k},\nonumber\\
	&\mathrm{with~} 0\leq\delta<\stimes\nonumber
\end{align}
\begin{equation}
	\label{eq:inputconst}
	\artinput\uli{i, \mathrm{min}} \leq \artinput\uli{i, \ell|k} \leq \artinput\uli{i, \mathrm{max}}, \forall\ell\in\left\{0,...,h\ul{s}-1\right\}
\end{equation}
%\begin{equation}
%	\label{eq:stateconst}
%	\begin{split}
%	&\posset{i}{}_{\mathrm{min}} < \posset{i}\of{kT + \kappa\stimecons + T|kT} < \posset{i}{}_{\mathrm{max}}\\
%	&\speedset{i}{}_{\mathrm{min}} < \speedset{i}\of{kT + \kappa\stimecons + T|kT} < \speedset{i}{}_{\mathrm{max}}\\
%	& \vey\uli{i, \mathrm{set}}{}_{\mathrm{min}} < \vey\uli{i, \mathrm{set}}\of{kT + \kappa\stimecons + T|kT} < \vey\uli{i, \mathrm{set}}{}_{\mathrm{max}}\\
%	 &\frac{\stimecons}{T} = \frac{H}{h\ul{const}}\in\mathbb{N}\text{,~} 0\leq \kappa \leq h_{const}
%	\end{split}
%\end{equation}
\begin{equation}
	\label{eq:stateconst}
	\begin{split}
	\vexset{i}{}_{,\mathrm{min}} \leq \vexset{i}\of{\kappa\stimecons + T|kT} \leq \vexset{i}{}_{,\mathrm{max}}~
	\forall\kappa\in \{0,...,h\ul{b}\}
	\end{split}
\end{equation}
\begin{equation}
	\label{eq:feascond}
	\begin{split}
	\speedset{i}\of{HT+T|kT} = \ve{0},~
	\vey\uli{i}\of{HT+T|kT} = \ve{0}
	\end{split}
\end{equation}
\begin{equation}
	\label{eq:collisionconstr}
	\begin{split}
	\ma{A}\uli{i, j, \mathrm{c}}\begin{bmatrix}
		\posset{i}\of{T|kT}\\
		\posset{i}\of{\stimecol+T|kT}\\
		\vdots\\
		\posset{i}\of{h\ul{c}\stimecol+T|kT}
	\end{bmatrix} \leq \ma{b}\uli{i, j, \mathrm{c}},\\\forall j\in\{1,...,N\},~j\neq i,
\end{split}
\end{equation}
\end{subequations}
with $\tfrac{T}{\stimeobj} = \tfrac{h\ul{o}}{H},\tfrac{T}{\stimecons} = \tfrac{h\ul{b}}{H},\tfrac{T}{\stimecol} = \tfrac{h\ul{c}}{H}\in\mathbb{N}$.
The solution of the optimization problem results in input values of the linear system (\ref{eq:dynamics}) such that a quadratic term between the planned trajectory and the desired target $\vex\uli{i, \mathrm{target}}$, and of the input with positive definite weights $\ma{Q}\uli{i}$, $\ma{R}\uli{i}$ is minimized under several conditions. All conditions are time-discrete and the state is obtained using the solution of linear state space systems (\ref{eq:dynconst}).
The different sample times $\stimes, \stimeobj, \stimecons, \stimecol$ allow us to tune the time density of the constraints independent of the inter-round time $T$, which cannot be tuned freely, because it depends on $T\ul{calc}$ and $T\ul{com}$. The sample times are chosen such that the ends of communication rounds fall on sample time points and the corresponding horizons $h\ul{s}, h\ul{o}, h\ul{b}, h\ul{c}$ are chosen such that all last sample time points fall on the same time $HT$, with prediction horizon $H$. This is important to ensure recursive feasibility (\cite{Park2021}). Because of the delay of calculation and communication, the trajectory starts in the next step $(k+1)T$.
The inputs and states are limited to a minimum and maximum (\ref{eq:inputconst})--(\ref{eq:stateconst}) according to dynamic limits of the UAV. Equation (\ref{eq:feascond}) is important for the feasibility at the next sample time point $(k+1)T$ (\cite{Park2021}). The property $\artinput\uli{i}\of{\tau+T|kT} = \ve{0}$ for all $\tau\geq HT$ then leads to $\vexset{i}\of{\tau+T|kT} = \vexset{i}\of{HT+T|kT}$ for all $\tau\geq HT$. Thus, at the end of the horizon, the UAV stops and stays at its position $\posset{i}\of{HT+T|kT}$.

The last constraint (\ref{eq:collisionconstr}) ensures that the UAV does not collide with others. The matrices $\ma{A}\uli{i, j, \mathrm{c}}$ and $\ma{b}\uli{i, j, \mathrm{c}}$ are calculated using TV-BVC (\cite{TVBVC}), which Figure \ref{fig:constrComp} illustrates.
%In this work, we use TV-BVC (\cite{TVBVC}) as anti-collision method, which Figure \ref{fig:constrComp} visualizes. 
For every sample time point, the \cu\ calculates the difference vectors between UAV $i$'s and UAV $j$'s last planned trajectory for all $h\in\{0,..., h_\mathrm{c}\}$
 \begin{equation*}
	\begin{split}
\ve{n}\uli{ij}\of{h\stimecol+2 T|(k-1)T} =\ma{\Theta}&{}^{-1}[\posset{j}\of{h\stimecol +2T|(k-1)T} \\&- \posset{i}\of{h\stimecol+2T|(k-1)T}].
	\end{split}
\end{equation*}
%where we set $\posset{j}\of{\tau|kT} = \posset{j}\of{HT+T|(k-1)T}$ for $\tau\geq HT$.
Then a plane with the normal vector $\ve{n}\uli{ij}$ is spanned in the center between the UAVs positions. UAV $i$ has to stay on the plane's right side with distance of at least $0.5\hat{r}\ul{min}$
\begin{align}
	\ve{n}\uli{0, ij}\of{h\stimecol+2T|(k-1)T}{}^\transp
\ma{\Theta}&{}^{-1}\left[\posset{j}\of{h\stimecol+2T|(k-1)T}\right.\nonumber\\
&\left. - \posset{i}\of{h\stimecol+T|kT}\right]\nonumber\\ 	\label{eq:lincolconst}
\geq \frac{1}{2}(\hat{r}\ul{min} + ||\ve{n}\uli{ij}(h\stimecol+2T|(&k-1)T)||_2),
\end{align}
where $\ve{n}\uli{0, ij}=\frac{\ve{n}\uli{ij}}{\twonorm{\ve{n}\uli{ij}}}$ and $\hat{r}\ul{min} \geq r\ul{min}$. We will show how to select $\hat{r}\ul{min}$ such that (\ref{eq:col}) holds in Theorem \ref{th:anticollcont}. Combining (\ref{eq:lincolconst}) for all $h\in\{0,...,h\ul{c}\}$, leads to constraint (\ref{eq:collisionconstr}).

After the \cu\ has solved optimization problem (\ref{eq:opt}), it sends the calculated trajectory and inputs to the UAV and all other \cus\ via the wireless network. The UAV sets $\veu\uli{i}\of{\tau+kT} = \veu\uli{i}\of{\tau|kT}$ for $\tau\in[T, 2T)$.
In cases of no recalculation ($\gamma\uli{q i}\of{k}=0, \forall q$), the UAV reuses the previously planned trajectory
% by enhancing it with the last planned position 
similar to \cite{Cai2018}
%\begin{equation}
%	\label{eq:noopttrajplan}\vexset{i}\of{\tau|kT}= \begin{cases}
%			\vexset{i}\of{\tau+T|(k-1)T} \text{~if~} \tau<HT\\
%			\left[\posset{i}\of{HT+T |(k-1)T}, \ve{0}, \ve{0}\right]^\transp \text{~else}
%		\end{cases}.
%\end{equation}
\begin{align}
	\label{eq:noopttrajplan}\vexset{i}\of{t|kT}= 
		\vexset{i}\of{t+T|(k-1)T}\\
		\label{eq:nooptinputplan}
		\veu\uli{i}\of{t|kT}=\veu\uli{i}\of{t+T|(k-1)T}.
\end{align}
for all $t\geq T$
%\begin{equation}
%	\label{eq:nooptinputplan}
%\veu\uli{i}\of{\tau|kT}= \begin{cases}
%			\veu\uli{i}\of{\tau+T|(k-1)T} \text{~if~} \tau<HT\\
%			\ve{0} \text{~else}
%		\end{cases}.
%\end{equation}
%\begin{equation}
%	\label{eq:nooptinputplan}
%	\veu\uli{i}\of{\tau|kT}=\veu\uli{i}\of{\tau+T|(k-1)T}.
%\end{equation}
In both situations, replanning or reusing, 
the resulting trajectories are not closer than $\hat{r}\ul{min}$ at the sampling points.
\begin{lemma}
	\label{lem:colguar}
If $\twonorm{\ve{n}\uli{ij}\of{h\stimecol+2T|(k-1)T}} \geq\hat{r}\ul{min}$ for $i \neq j$ and $\forall h\in\{0,..., h\ul{c}\}$, 
and if (\ref{eq:collisionconstr}) holds for both $i$ and $j$ independent of $\gamma\uli{q i}\of{k}$ and $\gamma\uli{q j}\of{k}~\forall q\in\{1,...,M\}$, then
\begin{align}
	\label{eq:guaranticoll}
	\twonorm{\ma{\Theta}^{-1}\left[\posset{j}\of{h\stimecol+T|kT}-\posset{i}\of{h\stimecol+T|kT}\right]}\geq \hat{r}\ul{min}
\end{align} 
\end{lemma}
\begin{proof}
	If agent $j$'s trajectory is not recalculated ($\gamma\uli{q j}\of{k}=0, \forall q$), it is with $\tau = h\stimecol+T$:
	\begin{align*}
			&\twonorm{\ma{\Theta}^{-1}\left[\posset{j}\of{\tau|kT} - \posset{i}\of{\tau|kT}\right]} \\
			&=\twonorm{\ve{n}\uli{0, ij}\of{\tau+T|(k-1)T}}\\
			&\qquad\times\twonorm{\ma{\Theta}^{-1}\left[\posset{j}\of{\tau|kT} - \posset{i}\of{\tau|kT}\right]}\\ & \geq  \ve{n}\uli{0, ij}\of{\tau+T|(k-1)T}^\transp\ma{\Theta}^{-1}(\posset{j}\of{\tau|kT} - \posset{i}\of{\tau|kT}) \\ &=\ve{n}\uli{0, ij}\of{\tau+T|(k-1)T}^\transp\\
			&\qquad\times\ma{\Theta}^{-1}(\posset{j}\of{\tau+T|(k-1)T} - \posset{i}\of{\tau|kT})\\&\geq \frac{1}{2}(\hat{r}\ul{min} + \twonorm{\ve{n}\uli{ij}\of{\tau+T|(k-1)T}}) \geq\hat{r}\ul{min}.
	\end{align*}
	If $\exists q, \text{~s.t.~} \gamma\uli{q j}\of{k}=1$, we can follow the proof for Lemma 1 of \cite{Zhou2017}. Because (\ref{eq:collisionconstr}) also holds for $j$, we know that (\ref{eq:lincolconst}) is also fulfilled when $i$ and $j$ swap places. Adding it to (\ref{eq:lincolconst}), we get (using $\ve{n}\uli{ij} = -\ve{n}\uli{ji}$)
		\begin{align}
			&\ve{n}\uli{0, ij}\of{\tau+T|(k-1)T}^\transp\ma{\Theta}^{-1}\left[(\posset{j}\of{\tau+T|(k-1)T}\right. \nonumber\\&\qquad\left. - \posset{i}\of{\tau|kT})- (\posset{i}\of{\tau+T|(k-1)T} - \posset{j}\of{\tau|kT})\right]\nonumber\\ & = 
		\ve{n}\uli{0, ij}\of{\tau+T|(k-1)T}^\transp\ma{\Theta}^{-1}(\posset{j}\of{\tau|kT} - \posset{i}\of{\tau|kT}) \nonumber\\& \qquad+\twonorm{\ve{n}\uli{ij}\of{\tau+T|(k-1)T}}\nonumber\\
		& \geq 
			\hat{r}\ul{min} + \twonorm{\ve{n}\uli{ij}\of{\tau+T|(k-1)T}}.\nonumber
		\end{align}
	Canceling $\twonorm{\ve{n}\uli{ij}\of{\tau+T|(k-1)T}}$ on both sides and applying the Cauchy-Schwarz inequality to the right side, we get (\ref{eq:guaranticoll}). 
%	Both argumentations above can also be done if we swap $i$ and $j$.
\end{proof}
With this result, we can state:
\begin{theorem}
	\label{th:feas}
	If $\vexset{i}\of{t+T|(k-1)T}$ fulfills (\ref{eq:dynconst})--(\ref{eq:collisionconstr}) and if\\ $||\ve{n}\uli{ij}(h\stimecol+T|(k-1)T)||_2 \geq\hat{r}\ul{min}$ for all pairwise different UAVs $i\neq j$ and $\forall h\in\{0,...,h\ul{c}\}$, then the subsequent trajectory $\vexset{i}\of{t|kT}$ generated by (\ref{eq:noopttrajplan}) also fulfills the constraints, the optimization problem (\ref{eq:opt}) is feasible at the following timestep $kT$ and $\twonorm{\ve{n}\uli{ij}\of{h\stimecol+T|kT}} \geq\hat{r}\ul{min}$.
\end{theorem}
\begin{proof}
	We use techniques from the proof of Theorem 2 in \cite{Park2021}.
	Because trajectory $\vexset{i}\of{t|kT}$ generated by (\ref{eq:noopttrajplan}) is equal to $\vexset{i}\of{t+T|(k-1)T}$ and the time duration $T$ is an integer multiple of the constraint sample times, it fulfills (\ref{eq:dynconst})--(\ref{eq:feascond}) in the first part ($t\leq HT$). The second part of the trajectory for $t>HT$ fulfills those constraints too, because the UAV stays at its position. 
	%Also (\ref{eq:feascond}) holds true.
	
%	Every other UAV $j$ gets its trajectory at optimization time $(k-1)T$ from the solution of the optimization problem (\ref{eq:opt}) or (\ref{eq:noopttrajplan}). For the first case, Lemma \ref{lem:colguar} states that the trajectories $\posset{i/j}\of{t|(k-1)T}$ of the UAVs $i$ and $j$ are at least $\hat{r}\ul{min}$ apart from each other at sample times. If UAV $j$ is using  (\ref{eq:noopttrajplan}), the first part of its trajectory $\posset{i/j}\of{t|kT}$ stays the same and at time $t>kT+HT$, the trajectories $\posset{i}\of{t|kT}$ and $\posset{j}\of{t+T|(k-1)T}$ have the same position as at time $kT+HT$. Thus the Thus, the corresponding linear constraint in (\ref{eq:collisionconstr}) is fulfilled.
%	Because (\ref{eq:noopttrajplan}) fulfills all constraints of (\ref{eq:opt}), (\ref{eq:opt}) is feasible at $kT$.
%	
%	 and thus the corresponding linear constraint in (\ref{eq:collisionconstr}) holds
The positions $\posset{i}\of{t|kT}$ and $\posset{i}\of{t+T|(k-1)T}$ are also equal with the same argumentation as above. If we now set this into the left side of (\ref{eq:lincolconst}), the left side is equal to
 $||\ve{n}\uli{ij}(h\stimecol+2T|(k-1)T)||_2$, which is bigger than the right side of (\ref{eq:lincolconst}) $\forall h\in\{0,...,h\ul{c}\}$ due to the second condition of this theorem and because the UAV stops for $t\geq HT$. Thus, the constraint (\ref{eq:collisionconstr}) holds. Because (\ref{eq:noopttrajplan}) fulfills all constraints of (\ref{eq:opt}), (\ref{eq:opt}) is feasible at $kT$. The argumentation above also holds, if $i$ and $j$ swap places. Lemma \ref{lem:colguar} then states that $\twonorm{\ve{n}\uli{ij}\of{h\stimecol+T|kT}} \geq\hat{r}\ul{min}$.
%The first part of the trajectory $\posset{i}\of{t|kT}$ generated by (\ref{eq:noopttrajplan}) stays the same as $\posset{i}\of{t+T|(k-1)T}$ and at time $t>kT+HT$, the trajectories $\posset{i}\of{t|kT}$ and $\posset{j}\of{t+T|(k-1)T}$ have the same position as at time $kT+HT$. Therefore  $\posset{i}\of{t|kT}$ and $\posset{j}\of{t+T|(k-1)T}$ have a distance (scaled with $\ma{\theta}^{-1}$) of at least $\hat{r}\ul{min}$ at sample times and thus (\ref{eq:collisionconstr}) holds. (we use Lemma \ref{lem:colguar} where we temporarily set the trajectory $\posset{j}\of{\cdot|kT}$ equal to the trajectory of $\posset{j}\of{\cdot|(k-1)T}$, which happens when it is generated using (\ref{eq:noopttrajplan})).
%Because (\ref{eq:noopttrajplan}) fulfills all constraints of (\ref{eq:opt}), (\ref{eq:opt}) is feasible at $kT$. Lemma \ref{lem:colguar} then directly states that $\twonorm{\ve{n}\uli{ij}\of{h\stimecol+T|kT}} \geq\hat{r}\ul{min}$.
%	Because (\ref{eq:noopttrajplan}) fulfills all constraints of (\ref{eq:opt}), (\ref{eq:opt}) is feasible at $kT$.
%	
\end{proof}

It directly follows from the recursive nature of this theorem that as long as the initial trajectories fulfill the conditions, we can generate trajectories without any collisions at sample time points with sample time $\stimecol$ using (\ref{eq:opt}) or (\ref{eq:noopttrajplan}) at all times.
%This means that when a drone is scheduled for replanning, the \cu\ definitively finds a solution. and when a drone is not scheduled, it will remain on a collision-free path.
%
%In case the drone is allowed to reoptimize its trajectory, the optimization will find a feasible solution.
%\begin{corollary}
%	\label{cor:feas}
%		If $\vexset{i}\of{t|(k-1)T}$ fulfills (\ref{eq:dynconst}) - (\ref{eq:collisionconstr}), then the optimization problem (\ref{eq:objectfunc}) has a feasible solution.
%\end{corollary}
%\begin{proof}
%	From theorem \ref{th:feas}, it directly follows that (\ref{eq:noopttrajplan}) fulfills alls constraint and thus the optimizationis a feasible solution.
%\end{proof}
However, this does not guarantee that (\ref{eq:col}) is fulfilled and the UAVs do not collide. The trajectories might get too close in between the sample time points (\cite{Luis2019}). The following theorem states under which conditions the swarm is guaranteed to be collision free:
\begin{theorem} \label{th:anticollcont}
	If $\vex\uli{i}\of{t|-T}$ fulfills the conditions of Theorem (\ref{th:feas}), if $\vex\uli{i}\of{T|-T}=\vex(0)$,
	%	If $\vexset{i}\of{t+T|-T} = \vex\uli{i}\of{0}=[\posset{i}\of{0}, \ve{0}, \ve{0}]^\transp$, $\veu\uli{i}\of{t+T|-T}=\ve{0}$ for every UAV $i$,
	and if $\hat{r}\ul{min} - \dpmax{i}{\stimecol} -\dpmax{j}{\stimecol} \geq r\ul{min}$~$\forall i,j\in\{1,...,N\}, i\neq j$ with
		\begin{align}
			%\label{eq:dpmax}
			\nonumber
			\Delta\ve{p}\uli{i, \mathrm{max}}(\tilde{T})&= \max_{\vexset{i}\in[\vexset{i}{}_{,\mathrm{min}},\vexset{i}{}_{,\mathrm{max}}], \artinput\uli{i}\of{t}\in[\artinput\uli{i,\mathrm{min}},\artinput\uli{i,\mathrm{max}}], \tau\in\left[0;\tilde{T}\right]}\bigg[\\ ||\begin{bmatrix}
					\ma{\Theta} & \ma{0}
				\end{bmatrix} \big[(e&{}^{\ma{A}\uli{i}\tau}-1)\vexset{i} +\int_{0}^{\tau}e^{\ma{A}\uli{i}\tilde{\tau}}\ma{B}\artinput\uli{i}(\tau-\tilde{\tau})\diff\tilde{\tau}\big]||_2\bigg]\nonumber
		\end{align}
	as upper bounds of the maximum distance, the position can travel between two sample time points with a sample time $\tilde{T}$, then the UAV swarm fulfills (\ref{eq:col}). 
%If $\vex\uli{i}\of{t|-T}$ fulfills the conditions of Theorem (\ref{th:feas}), if $\vex\uli{i}\of{T|-T}=\vex(0)$.
%%	If $\vexset{i}\of{t+T|-T} = \vex\uli{i}\of{0}=[\posset{i}\of{0}, \ve{0}, \ve{0}]^\transp$, $\veu\uli{i}\of{t+T|-T}=\ve{0}$ for every UAV $i$,
%	and if $\hat{r}\ul{min} - \dpmax{i}{\stimecol} -\dpmax{j}{\stimecol} \geq r\ul{min}$, then the UAV swarm fulfills (\ref{eq:col}).
\end{theorem}
\begin{proof}
	Feasible solutions of the trajectory planning exist for every $k\geq0$ (Theorem \ref{th:feas}).
	 %$\dpmax{i}{\tilde{T}}$ describes an upper bound of the maximum distance the setpoint-position  can travel in the time between two collision constraint sample points, i.e.
	 We select $k, h\ul{c}\in\mathbb{N}$ and $0\leq\delta< \stimecol$ such that $h\ul{c}\stimecol<T$ and $t=kT+\mathcal{T}$ with $\mathcal{T}=h\ul{c}\stimecol+T+\delta$.
	  Using Theorem \ref{th:feas} we know that
	  \begin{equation*}
	  	\begin{split} &\twonorm{\ma{\Theta}^{-1}[\posset{i}\of{t}-\posset{j}\of{t}]}=\twonorm{\ma{\Theta}^{-1}[\posset{i}\of{\mathcal{T}|kT}-\posset{j}\of{\mathcal{T}|kT}]}\\
	  	&\geq\twonorm{\ma{\Theta}^{-1}[\posset{i}\of{h\ul{c}\stimecol+T|kT}-\posset{j}\of{h\ul{c}\stimecol+T|kT}]}\\&\qquad-\dpmax{i}{\stimecol}-\dpmax{j}{\stimecol}\\
	  	&\geq \hat{r}\ul{min}-\dpmax{i}{\stimecol}-\dpmax{j}{\stimecol}.
	  \end{split}
	\end{equation*}
\end{proof}
%This theorem states that as long as $\hat{r}\ul{min}$ has some safety distance to the critical distance $r\ul{min}$ and the sampling time of the anti-collision constraints $\stimecol$ is low enough, the drones will not collide.
Theorem \ref{th:anticollcont} is independent of the chosen ET. 
%For example, even for the illogical rule $\gamma\uli{pi}\of{k} = 0,\forall p, i, k$, which never triggers a replanning, the UAVs will not collide (In this case they will just stay at their initial positions forever). 
There are two reasons for this independence. First, the swarm must have collision-free initial trajectories for Theorem \ref{th:anticollcont} to hold. Second, each UAV can recursively generate collision-free trajectories with (\ref{eq:noopttrajplan}) without triggering. However, when a UAV's replanning is not triggered for $H$ consecutive times, it will stop and stay at a position which might not be its target position. The choice of the ET is thus important to quickly steer the UAVs into their targets.

\textbf{Priority based trigger rule.} As a possible trigger rule, we chose  PBT (\cite{PredictiveTriggering}). With PBT, every UAV gets assigned a priority $g\uli{i}\of{kT}$. Because all \cus\ have the same information due to the many-to-all communication architecture, they can calculate the priorities of all UAVs locally without any additional communication. \cu\ $q$ then replans the trajectory of the UAV with $q$-th highest priority. The choice of the priority and its parameters allow us to tune the selection of UAVs and thus the performance of the overall system. We chose the following priority:
\begin{equation}
	\label{eq:prio}
	\begin{split}
		g\uli{i}\of{kT} =& \alpha\uli{1}\twonorm{\ve{d}\uli{i, \text{target}}}+\alpha\uli{2}\Delta t\uli{i}\of{kT}\\- \alpha\uli{3}&\max\Big(\cos\of{\beta},\sum_{j\neq i}\xi\frac{\ve{d}\uli{i, \text{target}}^\transp\ve{d}\uli{ij}}{||\ve{d}\uli{i, \text{target}}||_2||\ve{d}\uli{ij}||_2}\Big),
	\end{split}
\end{equation}
where $\ve{d}\uli{ij} = \posset{j}\of{2T|(k-1)T}-\posset{i}\of{2T|(k-1)T}$, $\ve{d}\uli{i, \text{target}} = \pos\uli{i, \text{target}}-\posset{i}\of{2T|(k-1)T}$ and
$\xi=\max\left(0, ||\ve{d}\uli{i, \text{target}}||_2 \right.$ $- ||\left. \ve{d}\uli{ij}||_2\right)$. $\Delta t\uli{i}\of{kT}$ describes how long the trajectory of UAV $i$ was not replanned. $\alpha\uli{1}, \alpha\uli{2}, \alpha\uli{3}\geq 0$ are weights of the summands. The last term measures how many UAVs lie in a cone with angle $\pm\beta$ between the UAV $i$ and its target and how close they are (factor $\xi$). The more UAVs, the more likely $i$ will get blocked by others and thus replanning is ineffective.

%\begin{theorem}
%	\label{th:anticollcont}
%	Define 
%	\begin{equation}
%		\label{eq:dxmax}
%		\begin{split}
%			&\dxmax{i}{\tilde{T}}\\ &\medmath{= \max_{\vexset{i}\in(\ref{eq:stateconst}), \artinput\uli{i}\in(\ref{eq:inputconst}), \tau\in\left[0;\tilde{T}\right]}\twonorm{ (e^{\ma{A}\uli{i}\tau}-1)\vexset{i} +\int_{0}^{\tau}e^{\ma{A}\uli{i}\tau}\ma{B}\diff\tau\artinput\uli{i}}}
%		\end{split}
%	\end{equation}
%	and
%	\begin{equation}
%		\label{eq:dpmax}
%		\begin{split}
%			\dpmax{i}{\tilde{T}}&= \max_{\vexset{i}\in(\ref{eq:stateconst}), \artinput\uli{i}\in(\ref{eq:inputconst}), \tau\in\left[0;\tilde{T}\right]}\left[\right.\\ &\medmath{\left.\twonorm{\begin{bmatrix}
%						\ma{\theta} & \ma{0}
%					\end{bmatrix} \left[(e^{\ma{A}\uli{i}\tau}-1)\vexset{i} +\int_{0}^{\tau}e^{\ma{A}\uli{i}\tau}\ma{B}\diff\tau\artinput\uli{i}\right]}\right]}
%		\end{split}
%	\end{equation}
%	as upper bounds of the maximum distance the setpoint (position) can travel between to sample points with sampling time $\tilde{T}$.
%	Let assumptions \ref{as:tubeMPC} and \ref{as:stab} hold true.
%	Define $d\uli{i}$ such that $\left\{\ma{\theta}\ve{a}|a\in\mathcal{D}\uli{i}\right\}%\ma{\theta}\bigotimes\mathcal{D}\uli{i}
%	\subseteq\mathcal{B}\ul{d\uli{i}}(0)$.
%	%\footnote{We define $\ma{M}\bigotimes\mathcal{A}=\left\{\ma{M}\ve{a}|\ve{a}\in\mathcal{A}\right\}$}
%	If $\posset{i}\of{t|0} = \pos\uli{i}\of{0}$, $\speedset{i}\of{t|0} = \speed\uli{i}\of{0} = \ve{0}$, $\vey\uli{i, \mathrm{set}}\of{0} = \ve{0}$, $\vey\uli{i}\of{0} = \ve{0}$ for every UAV,
%	if $\twonorm{\ve{n}\uli{ij}\of{h\stimecol+T+kT|(k-1)T}} >\hat{r}\ul{min}$,
%	if $(\ref{eq:inputconst})\Rightarrow\artinput\uli{i, \ell}\in\artinputset\uli{i}$ , if $(\ref{eq:stateconst})\bigoplus\dxmax{i}{\stimecons}\subseteq\mathcal{X}\uli{i,\mathrm{set}}$, if $\hat{r}\ul{min} - \dpmax{i}{\stimecol} -\dpmax{j}{\stimecol} - d\uli{i} - d\uli{j} \geq r\ul{min}$ and if $\vex\uli{i, \mathrm{set}}\of{0}$ fulfills constraints (\ref{eq:stateconst}) and (\ref{eq:collisionconstr}) for every UAV $i$, then the multi-agent UAV system fulfills (\ref{eq:col}).
%\end{theorem}
%\begin{proof}
%	Because of assumption \ref{as:stab} and theorem \ref{th:feas}, feasible solutions of the trajectory planning exist for every $k>0$.
%	%$\dpmax{i}{\tilde{T}}$ describes an upper bound of the maximum distance the setpoint-position  can travel in the time between two collision constraint sample points, i.e.
%	Because of theorem \ref{th:colguar} we know that $\twonorm{\ma{\theta}^{-1}[\posset{i}\of{t}-\posset{j}\of{t}]}>\hat{r}\ul{min}-\dpmax{i}{\stimecol}-\dpmax{i}{\stimecol}$.
%	Further the difference between the system trajectory $\vex\uli{i}\of{t}$ and $\vexset{i}\of{t}$ is always in $\mathcal{D}\uli{i}$ (see assumption \ref{as:tubeMPC}), i.e., the second order norm of this difference is always smaller equal $d\uli{i}$. Thus if $\hat{r}\ul{min} - \dpmax{i}{\stimecol} -\dpmax{j}{\stimecol} - d\uli{i} - d\uli{j} \geq r\ul{min}$, the trajectories always have a distance greater than $r\ul{min}$.
%\end{proof}

%While (\ref{eq:dxmax}) and (\ref{eq:dpmax}) can get calculated, 
%Applying this theorem formally will be very difficult or impossible for complex system dynamics, because of assumption \ref{as:tubeMPC}. However, from an engineer's point of view, this theorem states that as long as the sampling rates are high, the local controller allows the UAV to follow the setpoints closely and $\hat{r}\ul{min}$ has some safe distance to the critical distance $r\ul{min}$, the UAVs will never collide.

%In order to solve the optimization problem using quadratic programming, (\ref{eq:dynconst}) and (\ref{eq:discretisation}) are resolved using the time solution of linear systems.
%\begin{equation}
%	\begin{split}
%		&\vex\uli{i, set}\of{kT+\kappa\stimes+T+\delta|kT}\\
%		& = e^{\ma{A}\uli{i}(\kappa\stimes+\delta)}\vex\uli{i, set}\of{kT + T|(k-1)T}\\
%		& + \sum_{\ell=0}^{\kappa}\int_{\ell\stimes}^{\kappa\stimes+\delta}e^{\ma{A}\uli{i}\tau}\ma{B}\diff\tau\vev\uli{i, \ell}
%	\end{split}
%\end{equation}
%Inserting this into all other equations leads to an optimization problem with quadratic objective function and linear equality and inequality constraints.

==> event_triggered_dmpc_necsys22 - Kopie/Experiments/Experiments.tex <==
\section{Experiments and Discussion}
\pgfplotsset{compat=1.5.1}
\begin{figure}
	\centering
	\begin{tikzpicture}[spy using outlines={rectangle, magnification=2.5,connect spies}]
		\begin{axis}[xlabel={$t$ in \SI{}{\second}}, ylabel={Mean distance to target in \SI{}{\meter}}, ylabel style={text width=2.5cm}, xmin=0, xmax=60, legend style={at={(0.98,0.98)},anchor=north east ,draw=black,fill=white,align=left, nodes={scale=0.5, transform shape}}, height=0.2\textwidth, width=0.45\textwidth]
			\addplot [color=blue] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal2_15.csv};
			%\addlegendentry{$N=15, M=10$};
			\addplot [color=red] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal2_20.csv};
			%\addlegendentry{$N=20, M=10$};
			\addplot [color=black!30!green] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal2_25.csv};
			%\addlegendentry{$N=25, M=10$};
			\addplot [color=cyan] table [x index = {0}, y index = {1}]  {plotData/NoETFinal_25.csv};
			%\addlegendentry{$N=25, M=25$};
			\addplot [color=blue, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal2_15.csv};
			\addplot [color=red, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal2_20.csv};
			\addplot [color=black!30!green, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal2_25.csv};
			
			\coordinate (spypoint) at (axis cs:25,0.2);
			\coordinate (spyviewer) at (axis cs:37,3);
			\spy[width=5cm,height=1cm] on (spypoint) in node [fill=white] at (spyviewer);
		\end{axis}
	\end{tikzpicture}

	\caption{Mean distance to target. \capt{Dashed lines show the results of ET-DMPC with PBT, while the solid lines represent the results of ET-DMPC with round-robin scheduler. Blue: $N=15, M=10$, Red: $N=20, M=10$, Green: $N=25, M=10$, Cyan: $N=25, M=25$. In the mean, PBT is faster and more UAVs reach their target (magnification).}}
	\label{fig:successrate}
\end{figure}
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[xlabel={$t$ in \SI{}{\second}}, ylabel={$\twonorm{\pos\uli{i, \text{target}}-\pos\uli{i}}\of{t}$ in \SI{}{\meter}}, xmin=0, xmax=50, legend style={at={(0.98,0.98)},anchor=north east ,draw=black,fill=white,align=left, nodes={scale=0.7, transform shape}}, height=0.25\textwidth, width=0.5\textwidth]
%			\addplot [color=blue] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal_10.csv};
%			\addlegendentry{$N=10$};
%			\addplot [color=red] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal_20.csv};
%			\addlegendentry{$N=20$};
%			\addplot [color=purple] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal_30.csv};
%			\addlegendentry{$N=30$};
%			\addplot [color=orange] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal_40.csv};
%			\addlegendentry{$N=40$};
%			\addplot [color=green] table [x index = {0}, y index = {1}]  {plotData/RoundRobinFinal_50.csv};
%			\addlegendentry{$N=50$};
%			\addplot [color=blue, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal_10.csv};
%			\addplot [color=red, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal_20.csv};
%			\addplot [color=purple, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal_30.csv};
%			\addplot [color=orange, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal_40.csv};
%			\addplot [color=green, dashed] table [x index = {0}, y index = {1}]  {plotData/EventTriggeringFinal_50.csv};
%		\end{axis}
%	\end{tikzpicture}
%	\caption{Mean distance to target. \capt{Dashed lines show the results of ET-DMPC with TV-BVC and PBT, while the solid lines represent the results of ET-DMPC with TV-BVC and round-robin scheduler. In the mean, event-triggering is faster. The dotted line shows the results for ET-DMPC with PBT and linearized relaxed constraints (\cite{Luis2019}).}}
%	\label{fig:successrate}
%\end{figure}
\begin{figure}
	\newcommand{\figwidth}{0.20\textwidth}
	\centering
	\begin{tikzpicture}
		\newcommand{\radiusplot}{0.1}
		\newcommand{\plotlinewidth}{1}
		\begin{axis}[name=plot1, xlabel={$x$ in \SI{}{\meter}}, ylabel={$y$ in \SI{}{\meter}}, xmin=-1.5, ymin=-1.5, xmax=1.5, ymax=1.5 ,legend style={at={(0.98,0.021)},anchor=south east ,draw=black,fill=white,align=left, nodes={scale=0.7, transform shape}}, height=\figwidth, width=\figwidth]
			\fill (axis cs:1, 1) circle [black, fill,radius=\radiusplot];
			\fill (axis cs:-1, 1) circle [black, fill,radius=\radiusplot];
			\fill (axis cs:-1, -1) circle [black, fill,radius=\radiusplot];
			\fill (axis cs:1, -1) circle [black, fill,radius=\radiusplot];
			\fill (axis cs:-1, 0) circle [black, fill,radius=\radiusplot];
			\fill (axis cs:1, 0) circle [black, fill,radius=\radiusplot];
			
			\draw[->, dashed, blue, line width=1](axis cs:-1, 1)--(axis cs:1, -1);
			\draw[->, dashed, red, line width=1](axis cs:1, 1)--(axis cs:-1, -1);
			
			\draw[->, dashed, purple, line width=1](axis cs:-1, 0)--(axis cs:1, 1);
			\draw[->, dashed, orange, line width=1](axis cs:1, 0)--(axis cs:-1, 0);
			
			\draw[->, dashed, green, line width=1](axis cs:-1, -1)--(axis cs:-1, 1);
			\draw[->, dashed, cyan, line width=1](axis cs:1, -1)--(axis cs:1, 0);
		\end{axis}
		\coordinate[right=0.5cm of plot1] (coord);
		%\coordinate[right=1cm of coord] (coord2);
		\begin{axis}[name=plot2, at=(coord), anchor=left of west, xlabel={$x$ in \SI{}{\meter}}, ylabel={$y$ in \SI{}{\meter}}, xmin=-1.5, ymin=-1.5, xmax=1.5, ymax=1.5 ,legend style={at={(0.98,0.02)},anchor=south east ,draw=black,fill=white,align=left, nodes={scale=0.7, transform shape}}, height=\figwidth, width=\figwidth]
%			\addplot [color=blue, line width=\plotlinewidth] table [x index = {0}, y index = {1}]  {plotData/Example0.csv};
%			\addplot [color=red, line width=\plotlinewidth] table [x index = {0}, y index = {1}]  {plotData/Example1.csv};
%			\addplot [color=purple, line width=\plotlinewidth] table [x index = {0}, y index = {1}]  {plotData/Example2.csv};
%			\addplot [color=orange, line width=\plotlinewidth] table [x index = {0}, y index = {1}]  {plotData/Example3.csv};
%			\addplot [color=green, line width=\plotlinewidth] table [x index = {0}, y index = {1}]  {plotData/Example4.csv};
%			\addplot [color=cyan, line width=\plotlinewidth] table [x index = {0}, y index = {1}]  {plotData/Example5.csv};
%			\fill (axis cs:1, 1) circle [black, fill,radius=\radiusplot];
%			\fill (axis cs:-1, 1) circle [black, fill,radius=\radiusplot];
%			\fill (axis cs:-1, -1) circle [black, fill,radius=\radiusplot];
%			\fill (axis cs:1, -1) circle [black, fill,radius=\radiusplot];
%			\fill (axis cs:-1, 0) circle [black, fill,radius=\radiusplot];
%			\fill (axis cs:1, 0) circle [black, fill,radius=\radiusplot];
\addplot [color=blue, line width=\plotlinewidth] table [x index = {0}, y index = {1}]  {plotData/ExperimentPosition.csv};
\addplot [color=blue, line width=\plotlinewidth, dotted] table [x index = {0}, y index = {1}]  {plotData/ExperimentTargetPosition.csv};
\addplot [color=red, line width=\plotlinewidth] table [x index = {3}, y index = {4}]  {plotData/ExperimentPosition.csv};
\addplot [color=red, line width=\plotlinewidth, dotted] table [x index = {3}, y index = {4}]  {plotData/ExperimentTargetPosition.csv};
\addplot [color=purple, line width=\plotlinewidth] table [x index = {6}, y index = {7}]  {plotData/ExperimentPosition.csv};
\addplot [color=purple, line width=\plotlinewidth, dotted] table [x index = {6}, y index = {7}]  {plotData/ExperimentTargetPosition.csv};
\addplot [color=orange, line width=\plotlinewidth] table [x index = {9}, y index = {10}]  {plotData/ExperimentPosition.csv};
\addplot [color=orange, line width=\plotlinewidth, dotted] table [x index = {9}, y index = {10}]  {plotData/ExperimentTargetPosition.csv};
\addplot [color=green, line width=\plotlinewidth] table [x index = {12}, y index = {13}]  {plotData/ExperimentPosition.csv};
\addplot [color=green, line width=\plotlinewidth, dotted] table [x index = {12}, y index = {13}]  {plotData/ExperimentTargetPosition.csv};
\addplot [color=cyan, line width=\plotlinewidth] table [x index = {15}, y index = {16}]  {plotData/ExperimentPosition.csv};
\addplot [color=cyan, line width=\plotlinewidth, dotted] table [x index = {15}, y index = {16}]  {plotData/ExperimentTargetPosition.csv};
\fill (axis cs:1, 1) circle [black, fill,radius=\radiusplot];
\fill (axis cs:-1, 1) circle [black, fill,radius=\radiusplot];
\fill (axis cs:-1, -1) circle [black, fill,radius=\radiusplot];
\fill (axis cs:1, -1) circle [black, fill,radius=\radiusplot];
\fill (axis cs:-1, 0) circle [black, fill,radius=\radiusplot];
\fill (axis cs:1, 0) circle [black, fill,radius=\radiusplot];
		\end{axis}
	\end{tikzpicture}
	%\includegraphics[width=\linewidth]{pictures/BVC.pdf}
	\caption{Changing positions. \capt{The left plot shows which UAV has to fly to which position. The algorithm is able to lead all UAVs to their target position (right plot). Dotted lines are planned, solid lines real trajectories.}}
	\label{fig:circlechange}
\end{figure}
{\bf Simulation environment.} To evaluate the proposed methods, we have built a simulation of the system\footnote{The code with all parameters can be found in \url{https://github.com/Data-Science-in-Mechanical-Engineering/ET-distributed-UAV-path-planner}.}. It simulates a swarm of Crazyflies using gym-pybullet-drones
(\cite{panerati2021learning}). We approximate the quadcopter dynamics as a triple integrator for the DMPC (\cite{Wang2021}). Because it does not represent the real quadcopter dynamics accurately, the predicted positions using the linear model are set as setpoints of local position controllers of the UAVs (\cite{Luis2019}). We chose a sampling time of $T=\SI{333.33}{\milli\second}$ ($T\ul{calc}=\SI{233.33}{\milli\second}$, $T\ul{com}=\SI{100}{\milli\second}$). We set the minimal distance $\hat{r}\ul{min}=\SI{0.7}{\meter}$ and $\theta=\diag[1, 1, 2]$. %and define a drone crash, when the UAV's distance is lower than $r\ul{min} = \SI{0.2}{\meter}$. This difference of $\SI{0.5}{\meter}$ is chosen such that the deviation of the UAV to its setpoints does not lead to a collision.
The space where the UAVs can fly is limited to a cuboid of $\SI{5}{\meter}\times\SI{5}{\meter}\times\SI{5}{\meter}$. 
Initial and target positions are generated randomly using a truncated uniform random distribution such that initial/target positions scaled with $\ma{\theta}$ are not closer to each other than $\hat{r}\ul{min}$. We call one realization of initial and target positions scenario in the following. We could fit up to 25 UAVs in the space.

%To show the importance of feasibility and collision avoidance guarantees, we compare TV-BVC to linearized relaxed constraints (LRC, \cite{Luis2019}), which have no guarantees. We simulated 25 UAVs with 1000 scenarios for LRC and TV-BVC each and used PTB as ET. As seen in figure \ref{fig:successrate}, LRC allows the drones do reach their target faster in the mean. TODO only plot drones which have not crashed. However, it caused at least two UAVs to collide in \SI{29.6}{\percent} of all scenarios. In contrast, TV-BVC never lead to any collision. This shows that in high density swarms, the lack of guarantees leads to a high crash probability.

{\bf Influence of ET.} To determine the influence of ET, we compare PBT to a round-robin trigger. Figure \ref{fig:successrate} shows experiments with 15, 20 and 25 UAVs for $M=10$ \cus\ and TV-BVC with 1000 scenarios for each setup. In all setups, PBT steered the UAVs faster to their targets than round-robin. Additionally, the number of UAVs reaching their target is higher for PBT (\SI{98.5}{\percent}) than round-robin (\SI{92.7}{\percent}). But PBT cannot avoid completely that some UAVs are not able to reach their target.
This phenomenon is called deadlock
and caused by the absence of a centralized coordinator (\cite{Luis2019, Park2021}). Every UAV's trajectory is just optimal regarding the corresponding UAV. It thus would not make room for another UAV if this trajectory moved away from the target position. We noticed that some deadlocks lead to infeasibility due to numerical issues of the solver, which also hinders to dissolve them. Soft constraints could help to avoid this issue (\cite{Luis2019}). To avoid deadlocks completely, the targets $\pos\uli{i, \mathrm{target}}$ itself can be changed using a cooperative planner (\cite{Park2021}).

Furthermore, we compared the performance of a swarm with an equal number of UAVs and \cus\ ($N=M=25$) to one with less \cus\ than UAVs ($M=10<N=25$). We noticed that although some UAVs reached their target faster, there were a lot of deadlocks for $M=25$. This leads to the shape of the mean distance to target in Figure \ref{fig:successrate}. 
%In the first few seconds, the mean decreases fast, while it remains bigger than zero afterwards. 
Thus, in this scenario, ET not only saves \SI{60}{\percent} of bandwidth and computing hardware, it also improves the performance in the mean.

%Furthermore, we compared the performance of a swarm with equal number of UAVs and \cus\ ($N=M=25$) to one with less \cus\ than UAVs ($M=10<N=25$). As showed in figure \ref{fig:successrate}, using 25 \cus, the UAVs are faster reaching their target. In more realistic scenarios, e.g. delivery tasks, where only some UAVs are flying towards a target, the the performance gap might be smaller. The comparison shows that there is a trade-off between performance and bandwidth/expense savings, when choosing the number of \cus,  
%
%To show the effect of TV-BVC
%Figure \ref{fig:successrate} shows the results of our simulation. We simulated every setup 100 times and with ten \cus.
%
% 
%We evaluate the proposed methods on a swarm of Crazyflies. This is done in two ways. First an offline simulation based on \texttt{gym-pybullet-drones} (\cite{panerati2021learning}), second a hardware-in-the-loop (HiL) simulation with real Crazyflies, a simulated wireless network and simulated \cus running on a single PC based on Crazyswarm (\cite{Crazyswarm}). For the simulation, we use a four-times integrator and for the HiL-simulation a three-time integrator as linear model for the MPC\footnote{The code with all parameters can be found in \url{https://github.com/Data-Science-in-Mechanical-Engineering}.}. Because the real UAV's dynamics differ from the linear model, the predicted positions using the linear model are set as a setpoints of local position controller of the drones.
%For both, we set a sampling time of $T=\SI{333.33}{\milli\second}$. The sampling time is chosen because the optimization on the computers used takes less than $T\ul{calc}=\SI{233.33}{\milli\second}$ and the communication round is simulated to take $\SI{100}{\milli\second}$, which is based on former experiments with Mixer (\cite{PredictiveTriggering}).
%
%Figure \ref{fig:successrate} shows the results of our simulation. We simulated the system 10,000 times for different swarm sizes (1000 simulations per swarm size) and ten \cus. The space where the UAVs can fly is limited to a cuboid of $\SI{4.5}{\meter}\times\SI{4.5}{\meter}\times\SI{4.25}{\meter}$. Initial and target positions are generated randomly using a uniform random distribution such that initial and target positions scaled with $\ma{\theta}$ are not closer than $\SI{0.25}{m}$. We compare TV-BVC to linearized relaxed constraints (LRC, \cite{Luis2019}) and PBT to a round-robin scheduler. \SI{5}{\percent} of all drones crashed in our experiment with $N=50$ UAVs and LRC. Additional we noticed feasibility issues of the ET-DMPC with LRC. Tuning its parameters might improve the performance. However, feasibility and crash issues will never be resolved completely. In contrast, using TV-BVC only 0.01\% of the drones crashed and we observed no feasibility issues. We suppose that the DSLPID-controller included in  \texttt{gym-pybullet-drones} is not able to keep the UAV close to te trajectory in some scenarios. However, the proposed TV-BVC still leads to a much lower crash rate than LRC. In the experiments, swarms using LRC reached their target faster than TV-BVC. This is due to less conservative constraints, but with the higher probability of crashes.
%%It can be seen that most UAVs are able to reach their target after some time using ET-DMPC with TV-BVC. 
%%The more UAVs, the longer they need to reach their target. 
%%Because our method ensures collision free trajectories, in none of our experiments the UAVs crashed. When we used linearized relaxed constraints (\cite{Luis2019}) instead of TV-BVC, \SI{5}{\percent} of all drones crashed in our experiment with $N=50$. Additional we noticed feasibility issues of the DMPC with linearized relaxed constraints. Tuning its parameters might improve the performance, while TV-BVC guarantee feasibility and no collisions independent of the choice of parameters.
%
%For both, PBT and round-robin, most UAVs using ET-DMPC with TV-BVC are able to reach their target after some time.
%With PBT, UAVs reach their targets faster in the mean. In the first seconds, round robin is able to lower the mean distance to target faster. At some time, PBT overtakes round robin and the mean distance to target reaches $0$ faster. This may be due to round robin scheduling drones, which already reached their targets or are very close. PBT first brings all UAVs near their targets and then stears the UAVs into them.
% However, we noticed that event-triggering is faster than round-robin in not all evaluated initial/target state combinations. In more realistic scenarios, e.g. delivery tasks, only some UAVs try to reach targets. Then round-robin will assign resources to UAVs that do not need them. This will widen the performance gap between PBT and round-robin.
% %We noticed that the third summand in equation (\ref{eq:prio}) is important. Setting $\alpha\ul{3}=0$ leads to a worse performance of PBT than round-robin. 
%A small number of UAVs are not able to reach the target, because other UAVs block them. For PBT, this happened in \SI{0.13}{\percent} of all experiments.

{\bf Hardware-in-the-loop experiments.} To validate the sufficiency of the choice of a linear model for quadcopter trajectory generation, we tested our method using a hardware-in-the-loop (HiL) simulation with six real Crazyflies flying indoor. We  simulated the wireless network and one \cu\ on a local PC, which runs Crazyswarm (\cite{Crazyswarm}) and is connected to a motion capture system to obtain the positions of the crazyflies.
Figure \ref{fig:circlechange} shows an example trajectory of our HiL-simulation, where UAVs swap positions. We observed no dangerous flight maneuver and unstable behavior of the quadcopters when following the trajectory as can be seen in \url{https://youtu.be/2UzqOnUJQCA}. The choice of a linear model in our ET-DMPC seems to be sufficient for real quadcopters.

%Rarely occurring events in real quadcopter swarms, like technical failures or gusts, may cause a large difference between generated and real trajectory.
%In environments, where these events can occur, we suggest to use an additional event trigger. It should set the current setpoint to the real state (\cite{Luis2020, Park2021}), if their difference is too big. However, the event might lead to collisions or infeasibilities of the DMPC in this case. 


%\section{Discussion}
%\label{sec:disc}
%Although the experiments have shown that quadcopters with nonlinear dynamics can follow the trajectories generated using a linear model, there is no guarantee that this might lead to stable behavior of the quadctopter in every scenario. If formal guarantees are required, we suggest designing an controller based on exact input-output linearization (\cite{Fritsch2012}), which transforms the nonlinear to linear dynamics.

%Rarely occurring events, like technical failures or gusts may cause a large difference between generated and real trajectory
%In environments, where these events can occur, we suggest to use an additional event trigger. It should set the current setpoint to the real state (\cite{Luis2020, Park2021}), if their difference is too large. Note that in this case the event might lead to collisions or infeasibility of the DMPC. 

%In the experiments some drones did not reached their target. While PBT have been able to steer much more UAVs to their targets than round-robin, \SI{2}{\percent} did not reach it. This phenomenon is called deadlock
%and caused by the absence of a centralized coordinator (\cite{Luis2019, Park2021}). Every UAV's trajectory is just optimal regarding the corresponding UAV. Thus an UAV will not make place for another UAV, if this trajectory would move away from the target position. Changing the targets itself using a cooperative planner as proposed by \cite{Park2021} the targets itself in combination with PBT might help to avoid deadlocks.

==> event_triggered_dmpc_necsys22 - Kopie/Introduction/Introduction.tex <==
\section{Introduction}
In the recent years, unmanned aerial vehicle (UAV) swarms have become larger and larger, reaching sizes from 50 up to 100 UAVs (\cite{Crazyswarm}). To find trajectories that do not lead to colliding UAVs for such big swarms poses a challenge for path planning algorithms. The planning usually requires a lot of computational power, which can either be centralized or distributed among the UAVs. In the first case, a stationary computer transmits the trajectories to the UAVs over a wireless network. In the latter, the UAVs calculate their paths on-board and have to exchange information among themselves over a wireless network.
Central model predictive control (MPC) approaches like \cite{Augugliaro2012} need no powerful processor on board of the UAV. This decreases weight and thus energy consumption of the UAV. However, they do not scale well with an increasing number of UAVs (\cite{Luis2019}) and expose the system to the potential risk of a whole system failure if the central computer fails (\cite{alzain2012cloud}). Distributed model predictive control (DMPC) based approaches have become increasingly popular (\cite{Zhou2017}, \cite{Luis2019}, \cite{Luis2020} \cite{Park2021}). First, they do not require any central node since all computations are done on the UAVs. Second, they scale well with increasing number of UAVs. However, the on-board processing needs computational capacity and thus increases weight, leading to a higher energy consumption of the UAVs. 
%Offloading this computation to one powerful central computer would again expose the system to the same risk in case of central node failure.

% Central approaches allow to plan the trajectories on a powerful central computer and therefore need no powerful processor on board of the UAV. This decreases weight and thus power consumption of the UAV. However, they do not scale well with an increasing amount of UAVs (\cite{Park2021}, TODO besseres CITE) and expose the system to the potential risk of a whole system failure if the central computer fails (\cite{alzain2012cloud}). Distributed optimization based approaches however, have become more and more popular in the recent years (\cite{Zhou2017}, \cite{Luis2019}, \cite{Luis2020} \cite{Park2021}). First, they do not require any central node, as all processing is done on the UAVs. Second, they scale well with increasing amount of drones. But, the on-board processing needs computational capacity and thus increases the weight, leading to a higher power consumption of the drones, which a central approach avoids.
This work uses the ``best of both'' and combines centralized and distributed features based on a novel event-triggered DMPC (ET-DMPC) design.
% Such a combination is currently understudied, but has the potential to create an economic and controllable system (\cite{Dorigo2021}).
 Our approach consists of multiple stationary computation units (CU, Figure \ref{fig:overview}). Every \cu\ is placed on the ground and has enough power to replan the trajectory of one UAV at a time. It shares the resulting trajectory with other \cus\ and the UAVs over a wireless network, leveraging recent advances in low-power wireless technology (\cite{PredictiveTriggering}). The UAVs then follow their respective
 trajectories. However, it is not viable to provide one CU for each UAV in the swarm, which makes the system more expensive and may exceed the available network bandwidth. We thus propose to use fewer \cus\ than UAVs and present an event-triggering (ET) mechanism that enables trajectory replanning for only a subset of UAVs at a time.
 
This approach has benefits over purely centralized or distributed approaches. First, the UAVs need less on-board computational power, which saves weight and reduces energy consumption. Second, in contrast to standard centralized approaches, it is more robust against failures, because a failure of one CU does not lead to a whole system failure, as the remaining CUs in combination with ET can still plan the paths of the UAVs.
%Second, the event-triggering saves computation resources and reduces network traffic.
%Different to passive redundancy, i.e. having multiple backup computers in a central approach, this active redundancy leads to economical efficiency of the system,. 
The presented ET-DMPC uses features from existing DMPCs and scales well with the size of the swarm.
In summary, this paper makes the following contributions:
%\begin{itemize}
%	\item A novel distributed event-triggered computing method for path planning of large UAV swarms ;
%	\item a new DMPC formulation based on existing DMPC approaches (\cite{Luis2019,Luis2020, Park2021}), which uses ET  and guarantees feasibility and collision free trajectories for UAVs with linear dynamics;
%	\item an experimental evaluation of the effect the ET has on the overall performance\footnote{A video of the method controlling a real quadcopter swarm can be found in \url{https://youtu.be/oHK7mQI5wV0}.}. 
%\end{itemize}  
\begin{itemize}
	\item A novel distributed computing method for path planning of large UAV swarms which uses ET for improved resource efficiency;
	\item a new ET-DMPC formulation based on existing DMPC approaches (\cite{Luis2019,Luis2020, Park2021});
	\item formal proofs of recursive feasibility and collision free trajectories for UAVs with linear dynamics;
	\item an experimental evaluation of the effect that the ET has on the overall performance\footnote{A video of the method controlling a real quadcopter swarm can be found in \url{https://youtu.be/2UzqOnUJQCA}.}. 
\end{itemize}  

\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{pictures/Overview.pdf}
	\caption{Proposed event-triggered distributed Model Predictive Control (ET-DMPC) setup for path planning of UAV swarms. \capt{The computation units (CU) solve an MPC problem. They transmit the solution to the UAVs. An event-trigger decides which UAV's paths are replanned.}}
	\label{fig:overview}
\end{figure}

==> event_triggered_dmpc_necsys22 - Kopie/Makros.tex <==
\newcommand{\fakepar}[1]{\vspace{1mm}\noindent\textit{#1.}}
\newcommand{\capt}[1]{\mdseries{\emph{#1}}}
\newcommand*{\matlab}{\textit{Matlab}}
\newcommand*{\simulink}{\textit{Simulink}}
\newcommand*{\purepursuit}{\textit{Pure Pursuit}}
\newcommand*{\carCup}[0]{\textit{Carolo-Cup}~}
\newcommand*{\ros}[0]{\textit{ROS2}~}
\newcommand*{\psaf}[0]{Projektseminar Autonomes Fahren~}
\newcommand*{\darpa}[0]{\textit{DARPA}~}
\newcommand*{\opencv}[1]{\textit{OpenCV}}

\newcommand*{\jt}{\textit{Jetson TX2}}
\newcommand*{\jpi}{\textit{SDK Manager}}

% Formeln
\newcommand*{\phil}{\ensuremath{\varphi_\textrm{L}}}
\newcommand*{\philmax}{\ensuremath{\varphi_\textrm{L,max}}}
\newcommand*{\dphilmax}{\ensuremath{\dot{\varphi_\textrm{L,max}}}}

% Definition für Vektor und Matizen
\newcommand*{\mat}[1]{{\ensuremath{\mathrm{\textbf{#1}}}}}
\newcommand*{\ma}[1]{{\ensuremath{\boldsymbol{\mathrm{#1}}}}}
\newcommand*{\mas}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand*{\ve}[1]{{\ensuremath{\boldsymbol{#1}}}}
\newcommand*{\ves}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}

\newcommand*{\AP}{\ensuremath{\mathrm{AP}}}
\newcommand*{\doti}{\ensuremath{(i)^\cdot}}

\newcommand*{\inprod}[2]{\ensuremath{\langle #1,\,#2 \rangle}}

% Problem mit Siunitx
%\newcommand*{\ul}[1]{\underline{#1}}

% gerades "d" (z.B. für Integral)
\newcommand*{\ud}{\ensuremath{\mathrm{d}}}

% normaler Text in Formeln
\newcommand*{\tn}[1]{\textnormal{#1}}

% nicht-kursive Schrift in Formeln
\newcommand*{\mrm}[1]{\ensuremath{\mathrm{#1}}}

% gerades "T" für Transponiert
\newcommand*{\transp}{\ensuremath{\mathrm{T}}}

% gerades "rg"
\newcommand*{\rang}{\ensuremath{\operatorname{rg}}}

% Für geklammerte Ausdrücke mit Index (Subscript)
% (einmal mit kursiven Index, einmal mit geradem Index)
\newcommand*{\grpsb}[2]{\ensuremath{\left(#1\right)_{#2}}}
\newcommand*{\grprsb}[2]{\ensuremath{\left(#1\right)_{\mathrm{#2}}}}

% Ableitungen und Integrale
% "normale" Ableitung (mit geraden "d"s)
\newcommand*{\normd}[2]{\ensuremath{\frac{\mathrm{d}#1}{\mathrm{d}#2}}}
\newcommand*{\normdat}[3]{\ensuremath{\left.\frac{\mathrm{d} #1}{\mathrm{d} #2}\right|_{#3}}}

% Materielle Ableitung
\newcommand*{\matd}[2]{\ensuremath{\frac{\mathrm{D} #1}{\mathrm{D} #2}}}
\newcommand*{\matdat}[3]{\ensuremath{\left.\frac{\mathrm{D} #1}{\mathrm{D} #2}\right|_{#3}}}

% Partielle Ableitung
\newcommand*{\partiald}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand*{\partialdat}[3]{\ensuremath{\left.\frac{\partial #1}{\partial #2}\right|_{#3}}}


% Transformationen
\newcommand*{\FT}[1]{\ensuremath{\mathfrak{F}\left\{#1\right\}}}
\newcommand*{\FTabs}[1]{\ensuremath{\left|\mathfrak{F}\left\{#1\right\}\right|}}
\newcommand*{\IFT}[1]{\ensuremath{\mathfrak{F}^{-1}\left\{#1\right\}}}
\newcommand*{\DFT}[1]{\ensuremath{\mathrm{DFT}\left\{#1\right\}}}
\newcommand*{\DFTabs}[1]{\ensuremath{\left|\mathrm{DFT}\left\{#1\right\}\right|}}
\newcommand*{\Laplace}[1]{\ensuremath{\mathfrak{L}\left(#1\right)}}
\newcommand*{\InvLaplace}[1]{\ensuremath{\mathfrak{L^{-1}}\left(#1\right)}}
\newcommand*{\invtrans}{\ensuremath{\quad\bullet\!\!-\!\!\!-\!\!\circ\quad}}
\newcommand*{\trans}{\ensuremath{\quad\circ\!\!-\!\!\!-\!\!\bullet\quad}}





% Manche textcomp-Zeichen funktionieren mit dem TU-Design nicht, diese können dann mit diesem
% Befehl gesetzt werden.
\newcommand*{\textcompstdfont}[1]{{\fontfamily{cmr} \fontseries{m} \fontshape{n} \selectfont #1}}

\newcommand*{\mlfct}[1]{\texttt{#1}}

\newcommand*{\UL}[2]{#1_\mathrm{#2}}
\newcommand*{\ULi}[2]{#1_{#2}}
\newcommand*{\dy}[0]{\dot{y}}
\newcommand*{\ddy}[0]{\ddot{y}}
\newcommand*{\receivedPower}[0]{\frac{A}{y^2+h^2}}
\newcommand*{\dD}[0]{\dot{D}}
\newcommand*{\tf}[0]{\UL{t}{f}}
\newcommand*{\umax}[0]{\UL{u}{max}}

\newcommand*{\x}[1]{\UL{x}{#1}}
\newcommand*{\xv}[0]{\ve{x}}
\newcommand*{\la}[1]{\UL{\lambda}{#1}}
\newcommand*{\ua}[0]{\UL{u}{+}}
\newcommand*{\ub}[0]{\UL{u}{-}}
\newcommand*{\Ht}[1]{\tilde{H}(#1)}
\newcommand*{\Dp}[0]{\UL{D}{p}}
\newcommand*{\Dm}[0]{\overline{\dot{D}}}
\newcommand*{\fdynamic}[0]{\UL{\ve{f}}{dynamic}(\ve{y}, u)}
\newcommand*{\fE}[0]{\UL{f}{E}(\ve{y}, u)}
\newcommand*{\fD}[0]{\UL{f}{D}(\ve{y}, u)}
\newcommand*{\vl}[0]{\UL{v}{l}}
\newcommand{\vex}[0]{\ve{x}}
\renewcommand*{\of}[1]{\left(#1\right)}
%\renewcommand*{\of}[1]{{}_{,#1}}
\newcommand*{\vexof}[1]{\vex\of{#1}}
\newcommand*{\vexul}[1]{\UL{\vex}{#1}}
\newcommand*{\vexulof}[2]{\UL{\vex}{#1}\of{#2}}
\newcommand*{\vexuli}[1]{\ULi{\vex}{#1}}
\newcommand*{\hatvexuli}[1]{\ULi{\hat{\vex}}{#1}}
\newcommand*{\vexuliof}[2]{\ULi{\vex}{#1}\of{#2}}
\newcommand*{\hatvexuliof}[2]{\ULi{\hat{\vex}}{#1}\of{#2}}
\newcommand*{\pcom}[0]{{P\ul{com}}}
\newcommand*{\pcomhat}[0]{\hat{P}\ul{com}{}}
\newcommand{\weight}[2]{w\uliof{#1}{#2}}
\newcommand{\history}[0]{\mathcal{E}}
\newcommand{\weighthat}[2]{\hat{w}\uliof{#1}{#2}}

\newcommand*{\veerr}[0]{\ve{e}}
\renewcommand*{\ul}[1]{_{\mathrm{#1}} }
\newcommand*{\uliof}[2]{_{#1}{\of{#2}}}
\newcommand*{\uli}[1]{_{#1} }
\newcommand*{\koop}[0]{\mathcal{K}}
\newcommand*{\koopt}[0]{\mathcal{K}^t}
\newcommand*{\gof}[1]{g\of{#1}}
\newcommand*{\gul}[1]{\ULi{g}{#1}}
\newcommand*{\gofxof}[1]{\gof{\vexof{#1}}}
\newcommand*{\phivexof}[1]{\phi\of{\vexof{#1}}}
\newcommand*{\veg}[0]{\ve{g}}
\newcommand*{\vegof}[1]{\ve{g}\of{#1}}
\newcommand*{\vegulof}[2]{\ve{g}_{\mathrm{#1}}\of{#2}}
\newcommand*{\vey}[0]{\ve{y}}
\newcommand*{\veyof}[1]{\vey\of{#1}}
\newcommand*{\veyul}[1]{\UL{\vey}{#1}}
\newcommand*{\tzero}[0]{\UL{t}{0}}
\newcommand*{\vepsi}[0]{\ve{\psi}}
\newcommand*{\vephi}[0]{\ve{\phi}}
\newcommand*{\veu}[0]{\ve{u}}
\newcommand*{\veuof}[1]{\veu\of{#1}}
\newcommand*{\veuul}[1]{\UL{\veu}{#1}}
\newcommand*{\vev}[0]{\ve{v}}
\newcommand*{\vevof}[1]{\vev\of{#1}}
\newcommand*{\vevul}[1]{\UL{\vev}{#1}}
\newcommand*{\xul}[1]{\ULi{x}{#1}}
\newcommand*{\aul}[1]{\UL{a}{#1}}
%\newcommand*{\bul}[1]{\UL{b}{#1}}
\newcommand*{\kul}[1]{\UL{k}{#1}}
\newcommand*{\uul}[1]{\ULi{u}{#1}}

\newcommand*{\maAuli}[1]{\ULi{\ma{A}}{#1}}
\newcommand*{\veeps}[0]{\ve{\epsilon}}
\newcommand*{\twonorm}[1]{||#1||_\mathrm{2}}

\newcommand*{\lambdamaxof}[1]{\UL{\lambda}{max}\of{#1}}
\newcommand*{\lambdaminof}[1]{\UL{\lambda}{min}\of{#1}}
% Problem mit Siunitx
%\newcommand*{\A}[0]{Method A\:}
\newcommand*{\B}[0]{Method B\:}
%\newtheorem{definition}{Definition}[section]

%\newcommand*{\q}{q_\ve{\theta}}

\newcommand*{\tensorflowprob}{\textit{Tensorflow-Probability}~}

\newcommand*{\EX}[0]{\mathbb{E}}
\newcommand*{\tr}[0]{\mathrm{Trace}}
\newcommand*{\var }[0]{\mathrm{Var}}
\newcommand*{\given}[0]{\;\middle|\;}
\newcommand*{\gpess}[0]{g\ul{pess}{}}
\newcommand*{\gopt}[0]{g\ul{opt}{}}
\newcommand*{\tveerr}[0]{\tilde{\veerr}}
\newcommand*{\ofs}[1]{\left[#1\right]}
%\newcommand*{\g}[1]{g\uli{#1}}
%\newcommand*{\e}[2]{%
%\ifthenelse { \equal {#2} {} }  %if short caption not specified, use long caption (no slant)
%{ \veerr\uli{#1} }   % if #2 == blank
%{ \veerr\uli{#1}\of{#2} }   % else (not blank)

%}

\newcommand*{\matA}[1]{\ma{A}\uli{#1}}
\newcommand*{\matGamma}[0]{\ma{\Gamma}}
\newcommand*{\matGammaOpt}[0]{\ma{\Gamma}\ul{opt}}

\newcommand*{\matQ}[1]{{\ma{Q}\uli{#1}}}
\newcommand*{\matP}[1]{\ma{P}\uli{#1}}
\newcommand*{\eps}[2]{\epsilon\uli{#1}\of{#2}}
\newcommand*{\alp}[2]{\alpha\uli{#1}\of{#2}}
\newcommand*{\pfail}[0]{P\ul{loss}}
\newcommand{\priority}[2]{g\uli{#1}\of{\errorest{#1#1}{#2}}}
\newcommand*{\diag}[0]{\text{diag}}
\newcommand*{\tp}[1]{\of{#1}}
\newcommand*{\state}[2]{\vex\uli{#1}\tp{#2}}
\newcommand*{\stateest}[2]{\hat{\vex}\uli{#1}\tp{#2}}
\newcommand*{\noise}[2]{\ve{w}\uli{#1}\tp{#2}}
\newcommand*{\processnoise}[2]{\ve{v}\uli{#1}\tp{#2}}
\newcommand*{\errart}[2]{\ve{\tilde{e}}\uli{#1}\tp{#2}}
\newcommand*{\errorest}[2]{\ve{e}\uli{#1}\tp{#2}}
\newcommand*{\barerrorest}[2]{\ve{\bar{e}}\uli{#1}\tp{#2}}
\newcommand*{\errorestmeas}[2]{\ve{e}\uli{#1, meas}\tp{#2}}
\newcommand*{\erroragents}[2]{\hat{\ve{e}}\uli{#1}\tp{#2}}
\newcommand*{\erroragentstotal}[2]{\underline{\hat{\ve{e}}}\uli{#1}\tp{#2}}
\newcommand*{\erroresttotal}[2]{\underline{\ve{e}}\uliof{#1}{#2}}
\newcommand*{\matB}[1]{\ma{B}\uli{#1}}
\newcommand*{\matV}[1]{\ma{V}\uli{#1}}
\newcommand*{\matVti}[1]{\ma{\tilde{V}}\uli{#1}}
\newcommand*{\matW}[1]{\ma{W}\uli{#1}}
\newcommand*{\matAT}[1]{\left(\ma{A}\uli{#1}^\transp\right)}
\newcommand*{\matF}[1]{\ma{F}\uli{#1}}
\newcommand*{\rec}[2]{\gamma\uli{#1}\tp{#2}}
\newcommand*{\Cov}{\mathrm{Cov}}
\newcommand*{\matAti}[1]{\tilde{\ma{A}}\uli{#1}}

\newcommand{\io}[1]{\Gamma\of{#1}}
\newcommand{\oi}[1]{\Lambda\of{#1}}

\newcommand{\matAd}[1]{\tilde{\mat{A}}\ul{d, \mathrm{#1}}}
\newcommand{\ri}[1]{{r\uli{#1}}}
\newcommand{\di}[1]{{d\uli{#1}}}
\newcommand{\nii}[1]{{n\uli{#1}}}
\newcommand{\deltai}[1]{\Delta\uli{#1}}
\newcommand{\betai}[1]{\beta\uli{#1}}
\newcommand{\alphai}[1]{\alpha\uli{#1}}
\newcommand{\zetai}[1]{\zeta\uli{#1}}
\newcommand{\lmax}[1]{\lambda\ul{max}\of{#1}}
\newcommand{\lmin}[1]{\lambda\ul{min}\of{#1}}
\newcommand{\unknown}[0]{\left(\cdot\right)}
\newcommand*{\kt}[0]{\tilde{k}}
\newcommand*{\nz}[0]{\ve{n}\ul{0}}
\newcommand*{\norm}[2]{||#1||_{#2}}
\newcommand*{\diff}[0]{\text{d}}

\newcommand{\dalpha}[0]{\delta\alpha}
\newcommand{\setS}[0]{\mathcal{S}}
\newcommand{\cone}[0]{c\ul{1}\of{\setS}}
\newcommand{\ctwo}[0]{c\ul{2}\of{\setS}}

\newcommand{\pos}[0]{\ve{p}}
\newcommand{\speed}[0]{\ve{v}}
\newcommand{\acc}[0]{\ve{a}}

\newcommand{\posset}[1]{\pos\uli{#1, \mathrm{set}}}
\newcommand{\speedset}[1]{\speed\uli{#1, \mathrm{set}}}
\newcommand{\accset}[1]{\acc\uli{#1, \mathrm{set}}}
\newcommand{\vexset}[1]{\vex\uli{#1, \mathrm{set}}}
\renewcommand{\posset}[1]{\pos\uli{#1}}
\renewcommand{\speedset}[1]{\speed\uli{#1}}
\renewcommand{\accset}[1]{\acc\uli{#1}}
\renewcommand{\vexset}[1]{\vex\uli{#1}}
\newcommand{\stimeobj}[0]{T\ul{o}}
\newcommand{\stimes}[0]{T\ul{s}}
\newcommand{\stimecons}[0]{T\ul{b}}
\newcommand{\stimecol}[0]{T\ul{c}}
\newcommand{\dxmax}[2]{\Delta\vexset{#1}{}\ul{max}\of{#2}}
\newcommand{\dpmax}[2]{\Delta\posset{#1}{}\ul{,max}\of{#2}}

\newcommand{\cu}{CU}
\newcommand{\cus}{CUs}
\newcommand{\artinput}{\ve{u}}
\newcommand{\artinputset}{\mathcal{u}}

==> event_triggered_dmpc_necsys22 - Kopie/Problem_Setting/Problem_Setting.tex <==
\section{Problem Setting}
As a key conceptual difference to the aforementioned works, we introduce an architecture with $M$ \cus\ to control $N\geq M$ UAVs (see Figure \ref{fig:overview}).
In the following, the task of the UAVs is to fly to target positions without colliding with each other. While the UAVs' on-board computers do not have enough computational power to solve a trajectory planning problem, every \cu\ has enough capacity to solve it for one UAV at a time. In order to share information, UAVs and \cus\ use a wireless network. In this work, we assume a perfect connection without any message loss. However, we assume that the network has limited bandwidth and some delay.

The problem considered in this work splits into three different subproblems.
First, we need to design a \textbf{communication architecture} to facilitate robust data exchange between multiple stationary CUs and mobile UAVs.
Second, we need to formulate the \textbf{DMPC} that runs on the \cus. In this paper, as done in related works (\cite{Zhou2017,Luis2019, Luis2020, Wang2021}), we assume that the dynamics of the UAVs can be modeled by a linear system. We also assume that they are able to hover, e.g. like multicopters or balloon-based robots. The overall dynamics are described as
\begin{equation}
	\label{eq:dynamics}
	\begin{split}
	\dot{\vex}\uli{i} &= 
	\begin{bmatrix}
		\dot{\pos}\uli{i}\\
		\dot{\speed}\uli{i}\\
		\dot{\vey}\uli{i}
	\end{bmatrix} = \begin{bmatrix}\ma{0}&\ma{I}\uli{3}&\ma{0}\\
	\ma{0}&\ma{A}\uli{22, i}& \ma{A}\uli{23, i}\\
	\ma{0}&\ma{A}\uli{32, i}& \ma{A}\uli{33, i}
\end{bmatrix}\begin{bmatrix}
\pos\uli{i}\\
\speed\uli{i}\\
\vey\uli{i}
\end{bmatrix} +\begin{bmatrix}
\ma{0}\\
\ma{B}\uli{2, i}\\
\ma{B}\uli{3, i}
\end{bmatrix}\veu\uli{i}\\
&=\matA{i}\vex\uli{i} + \matB{i}\veu\uli{i},
\end{split}
\end{equation}
where $\pos\uli{i}$ and $\speed\uli{i}$ describe the position and speed of the UAV, $\vey\uli{i}$ summarizes the rest of the statespace of UAV $i$ (e.g. acceleration, jerk). $\veu\uli{i, \mathrm{min}}\leq\veu\uli{i}\leq\veu\uli{i, \mathrm{max}}$ is the control input of the system.
Third, the swarm and the \cus\ need to decide which UAV's trajectory gets replanned using \textbf{ET}. Because the system has more UAVs than \cus, the ET has to take the exact number of \cus\ directly into account. 

The combination of the network, DMPC and ET should steer the UAVs to their targets $\vex\uli{i,\mathrm{target}}=[\pos\uli{i, \mathrm{target}},\ve{0}, \ve{0}]$. To maintain safety, they have to guarantee that the UAVs do not collide. For collision-free trajectories, we will require that the positions are never closer than $r\ul{min}$,
\begin{equation}
	\label{eq:col}
	\begin{split}
	\twonorm{\ma{\Theta}^{-1}\left[\pos\uli{i}\of{t}-\pos\uli{j}\of{t}\right]} \geq r\ul{min},\\ \forall t>0~\forall i,j\in\left\{1,...,N\right\}, i\neq j.
	\end{split}
\end{equation} Because some types of UAV need to maintain a higher distance in one direction, e.g. due to downwash, the coordinate system is scaled using a symmetric positive definite matrix $\ma{\Theta}$ (\cite{Luis2019, Luis2020, Park2021}).
Additionally, the whole system has to guarantee that the DMPC problem is feasible at all time. Otherwise, the UAVs might collide because the algorithm fails to find a trajectory.
 
%\section{Problem Setting}
%\label{sec:problemsetting}
%Figure \ref{fig:overview} shows the setup considered in this work.
%The UAV swarm consists of $N$ drones. These need to fly to target positions, which are given by a high-level task planner. The drone's computers do not have enough computational capacity to solve a path planning problem. Therefore the system has $M$ computational units (CU). Every \cu has enough computational power to solve the path planning problem for one drone at a time. The $N$ agents and $M$ computational units are connected over a wireless network. In this work, we assume a perfect network connection without any message loss. The network has a round based many-to-all communication protocol like Mixer (\cite{Mixer}), i.e. at the end of a round all messages, which were sent by agents, have arrived at all agents in the network. During the round, the UAVs send their current state and the \cu share their results of the path planning, which the corresponding UAVs save in a buffer on their local computer. 
%After the communication round, the \cus decide which \cu replans the path of which UAV. Because of the many-to-all protocol, all \cus have the same information and need no communication in between for the scheduling. Then, each unit replans the trajectory of its assigned drone. The maximum duration for the scheduling and replanning $T\ul{calc}$ is constant for every agent and time. After the duration $T\ul{calc}$, a new communication round starts. The combined duration between the starts of two rounds is $T$.
%
%We assume that a local controller controls the UAVs. The combined dynamics of the UAV and the controller can be described by
%\begin{equation}
%	\label{eq:nonlinear}
%	\dot{\vex}\uli{i} = 
%	\begin{bmatrix}
%		\dot{\pos}\uli{i}\\
%		\dot{\speed}\uli{i}\\
%		\dot{\vey}\uli{i}
%	\end{bmatrix} = \begin{bmatrix}
%	\speed\uli{i}\of{t}\\
%	\ve{f}\ul{1}\of{\pos\uli{i}, \speed\uli{i}, \acc\uli{i}, \vey\uli{i}, \veu\uli{i}, t}\\
%	\ve{f}\ul{2}\of{\pos\uli{i}, \speed\uli{i}, \acc\uli{i}, \vey\uli{i}, \veu\uli{i}, t}
%\end{bmatrix}
%\end{equation}
%where $\pos\uli{i}$ and $\speed\uli{i}$ describe the position and speed of the UAV, $\vey\uli{i}$ summarizes all other states of the UAV or the controller. $\veu\uli{i}=\ve{h}\uli{i}\of{\pos\uli{i, set}, \speed\uli{i, set}, \vey\uli{i, set}, t}$ describes the setpoints of the controller. $\vey\uli{i, set}$ does not have to mimic $\vey\uli{i}$, i.e. its dimension and physical meaning can be different. Note that in reality the controller and setpoints will be time-discrete. Then, this function also samples and holds the inputs, i.e. its output will remain constant for at least the sampling time $T\ul{c}$ of the controller. It does not have to take the full state into account. For position control it may be sufficient to only use position setpoints.
%
%The goal of the following algorithm is to find setpoint trajectories, with guaranteed absence of collisions
%between the UAVs. We define that in collision free trajectories, the positions of two drones are never closer than $r\ul{min}$
%\begin{equation}
%	\label{eq:col}
%	\twonorm{\ma{\theta}^{-1}\left[\pos\uli{i}\of{t}-\pos\uli{j}\of{t}\right]} > r\ul{min}, \forall t>0~\forall i,j\in\left[1,N\right], i\neq j.
%\end{equation}
%Because some drones need to maintain a higher distance in one direction, e.g. due to downwash, the coordinate system is scaled using a symmetric positive definite matrix $\ma{\theta}$ \cite{Luis2019, Luis2020, Park2021}.	
%
%In this work, we generate the setpoints of the controller $\vex\uli{i, set} = [\pos\uli{i, set}, \speed\uli{i, set}, \vey\uli{i, set}]^\transp$ using a linear system model, i.e. they fulfill
%\begin{equation}
%	\label{eq:linearmodel}
%	\dot{\vex}\uli{i, set} = \ma{A}\uli{i}\vex\uli{i, set} + \ma{B}\uli{i}\artinput\uli{i}
%\end{equation}
%where $\artinput\uli{i}$ is an artificial input describing the degrees of freedoms of the setpoint trajectory. 
%%We assume that $(\ma{A}\uli{i}, \ma{B}\uli{i})$ is fully controllable. $\vey\uli{i, set}$ does not need to have the same dimension as $\vey\uli{i}$. 
%%In Section xy, we $\dot{\vey}\uli{i, set}$ will have a dimension of zero.
%We assume that the linear model is sufficient enough to generate trajectories, such that the UAV's real position always stays near the setpoint. This is similar to assumptions made in tube MPC (e.g. Definition 1 in \cite{Lopez2019}).
%\begin{assumption}
%	\label{as:tubeMPC}
%	There exists a non-empty and compact set $\mathcal{X}\uli{i, set}\subseteq\mathbb{R}^{n\ul{set}}$ and non-empty and compact sets $\mathcal{D}\uli{i}\subseteq\mathbb{R}^3, \artinputset\uli{i}\subseteq\mathbb{R}^v$ with zero as inner point, such that if $\vex\uli{i, set}\of{t}\in\mathcal{X}\uli{i, set}$, if there exists $\artinput\uli{i}\of{t}\in\artinputset\uli{i}$ such that $\vex\uli{i, set}\of{t}$ fulfills (\ref{eq:linearmodel}), if $\pos\uli{i}\of{0} = \pos\uli{i, set}\of{0}$ and if $\speed\uli{i}\of{0}=\speed\uli{i, set}\of{0} = \ve{0}$, $\vey\uli{i, set}\of{0}=\ve{0}$, $\vey\uli{i}\of{0} = \ve{0}$,  then $\pos\uli{i}\of{t}-\pos\uli{i, set}\of{t}\in \mathcal{D}\uli{i}, \forall t>0$.
%\end{assumption}
%We can use this assumption to make statements about the UAV's real trajectory by looking at setpoint trajectories, which are generated using (\ref{eq:linearmodel}). This allows us to lift this nonlinear problem into a linear regime. Additional, as described later, the linear model leads to a convex optimization problem, which can be solved efficiently with a numerical solver.
%
%%However, it may not be possible to check if Assumption \ref{as:tubeMPC} is fulfilled in reality, because of complex aerodynamic effects of UAVs.
%
%We further assume that the UAV can remain at a position forever.
%\begin{assumption}
%	\label{as:stab}
%	If
%	\begin{equation}
%	\medmath{	\vexset{i}\of{0}=\begin{bmatrix}
%			\posset{i}\of{0}\\
%			\ve{0}\\
%			\ve{0}
%		\end{bmatrix} \text{~and~} 	\vex\uli{i}\of{0}=\begin{bmatrix}
%		\posset{i}\of{0}\\
%		\ve{0}\\
%		\ve{0}
%	\end{bmatrix}}
%	\end{equation}
%then for $\artinput\uli{i}\of{t} = \ve{0}$
%\begin{equation}
%	\medmath{
%	\vex\uli{i, \mathrm{set}}\of{t} = \begin{bmatrix}
%		\posset{i}\of{0}\\
%		\ve{0}\\
%		\ve{0}
%	\end{bmatrix} \text{~and~}\vex\uli{i}\of{t} = \begin{bmatrix}
%	\posset{i}\of{0}\\
%	\ve{0}\\
%	\ve{0}
%\end{bmatrix}  ~\forall t>0}.
%\end{equation}
%\end{assumption}
%This assumption is important to ensure feasibility of the following MPC problem. 
%For UAVs, which are able to hover, like multicopters, one might be able to find a linear system that fulfills assumptions \ref{as:tubeMPC} and \ref{as:stab}. Therefore, we focus on them in the following. For winged UAVs, these assumptions are not fulfilled.

==> event_triggered_dmpc_necsys22 - Kopie/Related_Work/Related_Work.tex <==
\section{Related Work}
Many DMPC based trajectory planners  (\cite{Zhou2017, Cai2018, Luis2019, Luis2020, Park2021}) have the same communication structure but differ in their use of constraints and UAV models. In this structure, every UAV $i$ has knowledge about the last planned path of all other UAVs. It uses them to creates pairwise anti-collision constraints between them and the new planned path of itself. These constraints are used in an optimization problem, whose solution is the new planned path. In a next step, all UAVs share their calculated paths over a communication network with all other UAVs. We build on the same structure and leverage features of prior work such as the communication structure and DMPC formulation, however, we add \cus\ with ET to save resources and combine existing techniques to guarantee recursive feasibility and collisions free trajectories. 
%Many-to-all protocols like Glossy (\cite{Ferrari2011}) or Mixer (\cite{Mixer}) allow to implement the communication and have been successfully used in control applications (\cite{FeedbackControlGoesWireless,PredictiveTriggering}). For these reasons, we will use the same structure in this work. 

Although our ET mechanism can be used to adapt existing DMPC approaches, we will combine constraints and UAV models from different works to create our own DMPC algorithm, which guarantees feasibility and collision-free trajectories.
In this work, we will use the approach of \cite{Luis2019} and \cite{Luis2020} to use a linear state space model and linear anti-collision constraints to generate a quadratic-programming problem (QP). However, the anti-collision constraints presented in \cite{Luis2019} do not guarantee collision free trajectories, because the pairwise constraints have common intersections (see Figure \ref{fig:constrComp}). 
%To overcome feasibility issues of the QP, the works introduce relaxation constraints, which might also lead to collisions. 
%But we will change the constraints in a way such that they guarantee no collisions and feasibility of the system without the need for any relaxation constraints.
One method, which guarantees collision free trajectories are Buffered Voronoi Cells (BVC). They restrict the positions of the agents to be in separated sets (\cite{Zhou2017}). However, for large swarms, these sets are small and lead to poor performance (\cite{Luis2020}).
To overcome this problem, \cite{Park2021} use time-variant constraints based on the convex hull property of Bernstein polynomials. These constraints ensure that there are no collisions along the entire continuous trajectory. \cite{TVBVC} present a similar approach, where BVC are varied at every sample point of the optimization problem. We build on their idea of time-variant BVC (TV-BVC) in this paper. 
Additional, we will use the idea of \cite{Park2021} to introduce additional constraints to ensure recursive feasibility.
Concurrent with this work, \cite{Chen2022} have developed a similar strategy using TV-BVC and additional constraints to ensure recursive feasibility. However, the approach does not use ET to lower the communication bandwidth and calculates the solution of the DMPC on the UAVs. 
%yet without event-triggering.

\cite{Cai2018} present an ET-DMPC for quadcopter swarms. The DMPC uses nonlinear dynamics but does not guarantee feasibility and collision free trajectories. The ET has multiple triggering conditions and triggers recalculation if at least one of them is fulfilled. However, none of the conditions takes the limited computation power directly into account. This approach is thus not suitable for our setup, because the \cus\ can only replan a fixed number of UAVs at once. 

%Thus, there exist scenarios, where all UAVs replan at once. This is not suitable for our setup, because the \cus\ can only replan a subset of all UAVs at once. 
%While the approach of \cite{Cai2018} is designed for nonlinear dynamics, we will focus on linear dynamics, but guarantee collision-free trajectories and feasibility and take the limited bandwidth and computational power directly into account. 
%\cite{Park2021} use an additional constraint to the optimization problem that ensures feasibility in all next timesteps. We will use it to guarantee feasibility of our approach. 
%Bernstein polynomials need additional equality constraints in the optimization problem to ensure $\mathcal{C}^m$-continuity of the trajectory. This increases the size of the QP-problem and slows down the numerical solver. Because state space models ensure continuity by nature, our approach uses them instead.
  
